On sensitivity value of pair-matched observational studies

An observational study may be biased for estimating causal effects by failing to control for unmeasured confounders. This paper proposes a new quantity called the "sensitivity value", which is defined as the minimum strength of unmeasured confounders needed to change the qualitative conclusions of a naive analysis assuming no unmeasured confounder. We establish the asymptotic normality of the sensitivity value in pair-matched observational studies. The theoretical results are then used to approximate the power of a sensitivity analysis and select the design of a study. We explore the potential to use sensitivity values to screen multiple hypotheses in presence of unmeasured confounding using a microarray dataset.

==> waste.tex <==
% \appendix

\begin{example}
  Consider the Beta family of score functions:
  \begin{equation}
    \label{eq:beta-score}
    \psi_{a,b}(u) = \frac{u^{a-1}(1-u)^{b-1}}{\mathrm{Beta}(a,b)},~a,b>0.
  \end{equation}
  \Cref{tab:beta-family} shows the approximate mean of $\kappa^{*}$ in
  \eqref{eq:kappa-star-mean} for three score functions in this
  family. When $b = 0.6$, the score function $\psi$ is unbounded at $u
  = 1$. These functions have excellent design sensitivity at $I = \infty$
  for normal error, but they perform poorly with finite sample. The choice $\psi_{2,1}$ is the Wilcoxon signed rank test and
  is dominated by $\psi_{4,1}$ in all three sample sizes when the
  error is normally distributed (light tail), and by $\psi_{4,2}$ when the error is
  $t$-distributed (heavy tail).

  \renewcommand{\tabcolsep}{4pt}
  \begin{table}[h]
    \centering
    \caption{Approximate mean of $\kappa^*$ for some choices of score
      function in the Beta family when the data $Y$ is generated from
      location shift of $0.5$ or $1$ and normal or $t$-distributed (2
      degrees of freedom) error.}
    \begin{tabular}{ll|ccc|ccc|ccc|ccc}
      \hline
      & & \multicolumn{3}{c|}{$\mathrm{N}(0.5,1)$} & \multicolumn{3}{c|}{$\mathrm{N}(1,1)$} & \multicolumn{3}{c|}{$t_2+0.5$} & \multicolumn{3}{c}{$t_2+1$} \\
      $a$ & $b$ & $I$=100 & $I$=500 & $I$=$\infty$ & $I$=100 & $I$=500 & $I$=$\infty$ & $I$=100 & $I$=500 & $I$=$\infty$ & $I$=100 & $I$=500 & $I$=$\infty$ \\
      \hline
      2 & 0.6  & $0.70$ & $0.76$ & $0.81$ & $0.89$ & $0.92$ & $0.95$ & $0.54$ & $0.62$ & $0.67$ & $0.68$ & $0.74$ & $0.80$ \\
      & 1  & $0.68$ & $0.72$ & $0.76$ & $0.87$ & $0.90$ & $0.92$ & $0.61$ & $0.65$ & $0.69$ & $0.75$ & $0.79$ & $0.83$ \\
      & 2  & $0.60$ & $0.65$ & $0.69$ & $0.80$ & $0.83$ & $0.86$ & $0.61$ & $0.65$ & $0.69$ & $0.75$ & $0.79$ & $0.82$ \\
      & 4  & $0.52$ & $0.58$ & $0.62$ & $0.69$ & $0.74$ & $0.78$ & $0.55$ & $0.61$ & $0.65$ & $0.69$ & $0.74$ & $0.78$ \\
      4 & 0.6  & $0.73$ & $0.80$ & $0.86$ & $0.93$ & $0.96$ & $0.98$ & $0.48$ & $0.58$ & $0.66$ & $0.61$ & $0.70$ & $0.77$ \\
      & 1  & $0.73$ & $0.78$ & $0.82$ & $0.92$ & $0.95$ & $0.97$ & $0.58$ & $0.64$ & $0.69$ & $0.72$ & $0.78$ & $0.82$ \\
      & 2  & $0.67$ & $0.71$ & $0.75$ & $0.88$ & $0.91$ & $0.93$ & $0.62$ & $0.67$ & $0.71$ & $0.78$ & $0.82$ & $0.85$ \\
      & 4  & $0.59$ & $0.64$ & $0.68$ & $0.80$ & $0.84$ & $0.87$ & $0.61$ & $0.66$ & $0.70$ & $0.77$ & $0.81$ & $0.84$ \\
      8 & 0.6  & $0.74$ & $0.83$ & $0.90$ & $0.94$ & $0.97$ & $0.99$ & $0.38$ & $0.52$ & $0.63$ & $0.50$ & $0.63$ & $0.73$ \\
      & 1  & $0.75$ & $0.82$ & $0.87$ & $0.95$ & $0.97$ & $0.99$ & $0.51$ & $0.60$ & $0.67$ & $0.65$ & $0.73$ & $0.79$ \\
      & 2  & $0.71$ & $0.77$ & $0.81$ & $0.93$ & $0.95$ & $0.97$ & $0.59$ & $0.66$ & $0.71$ & $0.75$ & $0.80$ & $0.84$ \\
      & 4  & $0.65$ & $0.70$ & $0.75$ & $0.88$ & $0.91$ & $0.94$ & $0.62$ &
      $0.68$ & $0.73$ & $0.78$ & $0.83$ & $0.87$ \\
      \hline
    \end{tabular}
    \label{tab:beta-family}

  \end{table}
\end{example}

Consider the sample splitting strategy which computes sensitivity
value $\kappa^{*}$ for
all the treatments/outcomes using $(1 - \zeta)$ proportion of the
sample, and then select all the treatments/outcomes with $\kappa^{*}$ greater than
some value $\tilde{\kappa}$. Finally, the sensitivity values computed
using the rest $\zeta$ proportion of the sample are reported. Notice
that in this procedure the sensitivity values in the first sample are determined with critical value $\tilde{\alpha}$ and in the second sample $\kappa^{*}$
are determined with $\alpha / |\mathcal{S}|$ to control the
family-wise error rate (FWER) at $\alpha$, where $\mathcal{H}$ is
all the hypotheses and $\mathcal{S}$ is the selected hypotheses (a
random set).

Using the power approximation \eqref{eq:power}, the false positive
rate of the screening step is given by
\begin{equation}
  \mathrm{FPR} = 1 - \Phi\Big( \frac{-\sqrt{(1-\zeta)I} (\mu_{F_0} - \tilde{\kappa}) + \sigma_q
    \bar{\Phi}^{-1}(\tilde{\alpha}) \sqrt{\mu_{F_0} (1 - \mu_{F_0})}}{\sigma_{F_0}}\Big),
\end{equation}
It is easy to verify that under the null $\mu_{F_0} = 1/2$ and $\sigma_{F_0} =
\sigma_q/2$. Similarly, the
false negative rate against a particular distribution $F$ is given by
\begin{equation}
  \mathrm{FNR} = \Phi\Big(\frac{-\sqrt{(1-\zeta)I} (\mu_F - \tilde{\kappa}) + \sigma_q
    \bar{\Phi}^{-1}(\tilde{\alpha})\sqrt{\mu_F(1-\mu_F)}}{\sigma_F}\Big).
\end{equation}
In principle, we would like to use the smallest sample size
$(1-\zeta)I$ to ensure that $\mathrm{FPR} \le
\alpha_{\mathrm{FP}}$ and $\mathrm{FNR} \le \alpha_{\mathrm{FN}}$ for
some small $\alpha_{\mathrm{FP}}$ and $\alpha_{\mathrm{FN}}$ (such as
0.05). Assuming $1/2 < \tilde{\kappa} < \mu_F$, this requires
\begin{equation} \label{eq:sample-size-lower-bound}
  \begin{split}
    \sqrt{(1-\zeta)I} \ge \max\Big\{ &\frac{\big[\bar{\Phi}^{-1}(\alpha_{\mathrm{FP}}) -
      \bar{\Phi}^{-1}(\tilde{\alpha})\big] \sigma_q/2}{\tilde{\kappa} - 1/2},~\frac{\sigma_{F}
      \bar{\Phi}^{-1}(\alpha_{\mathrm{FN}}) + \sigma_q \bar{\Phi}^{-1}(\tilde{\alpha})
      \sqrt{\mu_F(1-\mu_F)}}{\mu_F - \tilde{\kappa}} \Big\}.
  \end{split}
\end{equation}
The question is: what choice of $(\tilde{\alpha},\tilde{\kappa})$
minimizes the above lower bound?

\begin{theorem}
  For $\mu_F > 1/2$, the right hand side of
  \eqref{eq:sample-size-lower-bound} achieves its minimum at
  $\tilde{\alpha} = \alpha_{\mathrm{FP}}$ and $\tilde{\kappa} \to 1/2$.
\end{theorem}
\begin{proof}
  The first lower bound in \eqref{eq:sample-size-lower-bound} is increasing in
  $\tilde{\alpha}$ and
  decreasing in $1/2 < \tilde{\kappa} < 1$, and the second lower bound
  in \eqref{eq:sample-size-lower-bound} is increasing in $\tilde{\kappa}$ and decreasing in
  $\tilde{\alpha}$. Therefore their maximum is minimized when the two
  lower bounds are the same. For a fixed $\alpha_{\mathrm{FP}} <
  \tilde{\alpha}$, we can obtain the optimal $\kappa^{*}$ by equating
  the lower bounds. Plugging that expression back in, the right hand
  side of \eqref{eq:sample-size-lower-bound} becomes
  \[
  \frac{\sigma_{F}
    \bar{\Phi}^{-1}(\alpha_{\mathrm{FN}}) + \sigma_q \bar{\Phi}^{-1}(\tilde{\alpha})
    \sqrt{\mu_F(1-\mu_F)} + \big[\bar{\Phi}^{-1}(\alpha_{\mathrm{FP}}) -
    \bar{\Phi}^{-1}(\tilde{\alpha})\big] \sigma_q/2}{\mu_F - 1/2}.
  \]
  Since $\mu_F > 1/2$, $\sqrt{\mu_F (1 - \mu_F)} < 1/2$. Hence the above
  expression is an increasing function of $\tilde{\alpha}$. Therefore
  the optimal $\tilde{\alpha}$ is $\alpha_{\mathrm{FP}}$. In this case
  the false positive rate is always controlled. To maximizing the power
  of selecting non-null hypotheses, we should use the smallest
  $\tilde{\kappa}$ possible.
\end{proof}

This Theorem suggests that we only need to use the p-values under the
null ($\kappa = 1/2$) to screen hypotheses no matter what test
statistic we use.


% The next Theorem finds the optimal score function in finite sample.
% \begin{theorem} \label{thm:optimal-psi}
%   The optimal score function $\psi$ that maximizes the approximation
%   of $\mathrm{E}[\kappa^{*}]$ in \eqref{eq:kappa-star-mean} can be expressed as
%   \[
%   \psi(u) = \max(\beta g(u) - \gamma, 0).
%   \]
%   for some constants $\beta = \beta(\alpha,I) > 0$, $\gamma =
%   \gamma(\alpha,I) > 0$ that solves
% \[
% \frac{\sqrt{I}}{\bar{\Phi}^{-1}(\alpha)} = \frac{\beta\sqrt{\langle
%     \psi, g \rangle (1 - \langle \psi, g \rangle)}}{\|\psi\|_2} -
% \|\psi\|_2 \frac{2 \langle
%     \psi, g \rangle - 1}{\sqrt{\langle
%     \psi, g \rangle (1 - \langle \psi, g \rangle)}}
% \]
% \end{theorem}

% We apply this theory to the U-statistics developed in
% \citet{rosenbaum2011new}. Each U-statistic is parametrized by three
% integer numbers, $(m, \overline{m}, \underline{m})$ with $\underline{m}
% \le m \le \overline{m}$ and \citet[Lemma
% 1]{rosenbaum2011new} derives the limiting score function
% \[
% \psi(u) = \sum_{l = \underline{m}}^{\overline{m}} l {m \choose l}
% p^{l-1} (1 - p)^{m-l}.
% \]


%  the design sensitivity can be
% expressed as
% \[
% \begin{split}
%   \mu_{F_\theta} &= \int_0^{\infty} \psi\big(F(x-\theta) - F(-x-\theta)\big)
%   f_0(x-\theta) \diff x \\
%   &= \int_{-\theta}^{\infty} \psi\big(F(x) - F(-x-2\theta)\big)
%   f_0(x) \diff x.
% \end{split}
% \]
% \item

% \section{Proof of \Cref{thm:optimal-psi}}
% \label{sec:proof-crefthm:-psi}

% We solve this functional optimization problem
% using variational calculus. Consider an arbitrary function $\|v\|_1 =
% 1$, $v(u) \ge 0$. Let $\psi_{\epsilon}(u) = (1 -
% \epsilon) \psi(u) + \epsilon v(u)$. It is easy to show that
% $\|\psi_{\epsilon}(u)\|_1 = 1$ and $\psi_{\epsilon} \ge 0$ for
% sufficiently small $\epsilon$. The first variation of the functional
% $\mu_{F,I}$ is defined as
% \[
% \begin{split}
%   \delta_v (\mu_{F,I}[\psi]) = \lim_{\epsilon \to 0}
%   \frac{\mu_{F,I}[\psi_{\epsilon}] - \mu_{F,I}[\psi]}{\epsilon}
% \end{split}
% \]
% Since
% \[
% \langle \psi_{\epsilon}, g \rangle = \langle \psi, g \rangle +
% \epsilon\langle v - \psi, g \rangle,
% \]
% using the expansion $\sqrt{a+\epsilon} = \sqrt{a} +
% \epsilon/(2\sqrt{a}) + O(\epsilon^2)$ we get
% \[
% \begin{split}
%   \sqrt{\langle \psi_{\epsilon}, g \rangle (1 - \langle \psi_{\epsilon}, g \rangle)}
%   &= \sqrt{(\langle \psi, g \rangle +
%     \epsilon\langle v - \psi, g \rangle) (1 - \langle \psi, g \rangle -
%     \epsilon\langle v - \psi, g \rangle)} \\
%   &= \sqrt{\langle \psi, g \rangle (1 - \langle \psi, g \rangle)} +
%   \epsilon \cdot \frac{\langle v - \psi, g \rangle (1 - 2 \langle \psi,
%     g \rangle)}{2\sqrt{\langle \psi, g \rangle (1 - \langle \psi, g
%       \rangle)}} + O(\epsilon^2),
% \end{split}
% \]
% and
% \[
% \begin{split}
%   \|\psi_{\epsilon}\|_2 &= \sqrt{\int_0^1 (1 - \epsilon)^2 \psi^2(u) +
%     2\epsilon(1-\epsilon)\psi(u) v(u) + \epsilon^2 v^2(u) \diff u} \\
%   &= \|\psi\|_2 + \epsilon \cdot \frac{\langle v - \psi, \psi \rangle}{\|\psi\|_2} + O(\epsilon^2).
% \end{split}
% \]

% Using the above expansions, we can compute the first variation
% \[
% \begin{split}
%   \delta_v (\mu_{F,I}[\psi]) = \langle v - \psi, g \rangle -
%   \frac{\bar{\Phi}^{-1}(\alpha)}{\sqrt{I}} \bigg\{& \frac{\langle v - \psi,
%     \psi \rangle}{\|\psi\|_2} \sqrt{\langle \psi, g \rangle (1 -
%     \langle \psi, g \rangle)} \\ &+ \|\psi\|_2 \frac{\langle v - \psi, g
%     \rangle (1 - 2 \langle \psi,   g \rangle)}{2\sqrt{\langle \psi, g
%       \rangle (1 - \langle \psi, g    \rangle)}} \bigg\}.
% \end{split}
% \]

% Let $v(u) = \Delta_u$ be the Dirac delta function at $u$ and for
% notational simplicity denote $\langle \psi, g \rangle = b$, we get
% \begin{equation} \label{eq:delta-dirac-delta}
%   \begin{split}
%     \delta_{\Delta_u} (\mu_{F,I}[\psi]) = (g(u) - b) -
%     \frac{\bar{\Phi}^{-1}(\alpha)}{\sqrt{I}} \bigg\{ \frac{\psi(u) -
%       \|\psi\|_2^2}{\|\psi\|_2} \sqrt{b(1-b)} + \|\psi\|_2 \frac{(g(u)
%       - b) (1 - 2 b)}{2\sqrt{b(1-b)}} \bigg\}.
%   \end{split}
% \end{equation}
% A sufficient condition for $\psi$ maximizing $\mu_{F,I}[\psi]$ is that
% the first variation $\delta_v(\mu_{F,I}[\psi]) \le 0$ for any function $v$
% such that $\|v\|_1 = 1$, $v(u) \ge 0$. We can apply the same calculation to the variation
% $\tilde{\psi}_{\epsilon} = (1 + \epsilon) \psi(u) - \epsilon v(u)$ for
% an arbitrary function $v$ such that $\|v\|_1 = 1$, $v(u) \ge 0$ and
% $v(u) = 0$ if $\psi(u) = 0$.

% This implies that a sufficient condition
% for $\psi$ maximizing $\mu_{F,I}[\psi]$ is that
% \[
% \delta_{\Delta_u} (\mu_{F,I}[\psi]) \le 0,~\delta_{\Delta_u}(\mu_{F,I}[\psi]) = 0~\mathrm{if}~\psi(u) > 0.
% \]

% Therefore there exist constants
% $\beta = \beta(\alpha,I) > 0$, $\gamma = \gamma(\alpha,I) > 0$ such that
% \[
% \psi(u) = \max(\beta g(u) - \gamma, 0).
% \]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

